ParaGraph: Weighted Graph Representation for Performance Optimization of HPC Kernels

GPU-based HPC clusters are attracting more scientific application developers due to their extensive parallelism and energy efficiency. In order to achieve portability among a variety of multi/many core architectures, a popular choice for an application developer is to utilize directive-based parallel programming models, such as OpenMP. However, even with OpenMP, the developer must choose from among many strategies for exploiting a GPU or a CPU. Recently, Machine Learning (ML) approaches have brought significant advances in the optimizations of HPC applications. To this end, several ways have been proposed to represent application characteristics for ML models. However, the available techniques fail to capture features that are crucial for exposing parallelism. In this paper, we introduce a new graph-based program representation for parallel applications that extends the Abstract Syntax Tree to represent control and data flow information. The originality of this work lies in the addition of new edges exploiting the implicit ordering and parent-child relationships in ASTs, as well as the introduction of edge weights to account for loop and condition information. We evaluate our proposed representation by training a Graph Neural Network (GNN) to predict the runtime of an OpenMP code region across CPUs and GPUs. Various transformations utilizing collapse and data transfer between the CPU and GPU are used to construct the dataset. The predicted runtime of the model is used to determine which transformation provides the best performance. Results show that our approach is indeed effective and has normalized RMSE as low as 0.004 to at most 0.01 in its runtime predictions.

==> figures/augmentedAST_old.tex <==
\begin{figure*}[ht!]
\centering
\tikzset{
empty/.style = {ellipse, minimum width=2.5cm},
base/.style = {draw, ellipse, minimum width=2.5cm},
for/.style = {->, >=stealth, thick, purple},
legend/.style = {minimum width=2.5cm, anchor=west, text width=2.3cm},
}
\resizebox{\textwidth}{!} {
\scriptsize
\begin{tikzpicture}
    \node[base](csbo1) at (4.5,14.5) {CompoundStmt};
    \node[base](bobo1) at (4.5,13) {BinaryOperator};
    \node[base](icebo1) at (1.5,11.5) {ImplicitCastExpr};
    \node[base](inbo1) at (7.5,11.5) {IntegerLiteral};
    \node[base](varbo1) at (0,13.5) {VarDecl};
    \node[empty] at (2.25,13) {\textbf{. . .}};
    \node[base](drebo1) at (1.5,10) {DeclRefExpr};
    
    \draw[-] (csbo1) -- (bobo1);
    \draw[-] (bobo1) -- (icebo1);
    \draw[-] (bobo1) -- (inbo1);
    \draw[-] (icebo1) -- (drebo1);
	
	\draw[-implies,line width=1pt,double distance=5pt] (9,13) -- (11,13);
	
    \node[base](csbo1) at (16.5,14.5) {CompoundStmt};
    \node[base](bobo1) at (16.5,13) {BinaryOperator};
    \node[base](icebo1) at (13.5,11.5) {ImplicitCastExpr};
    \node[base](inbo1) at (19.5,11.5) {IntegerLiteral};
    \node[base](varbo1) at (12,13.5) {VarDecl};
    \node[empty] at (14.25,13) {\textbf{. . .}};
    \node[base](drebo1) at (13.5,10) {DeclRefExpr};
    
    \draw[-] (csbo1) -- node[pos=0.5, left] {1} (bobo1);
    \draw[-] (bobo1) -- node[pos=0.5, above left] {1} (icebo1);
    \draw[-] (bobo1) -- node[pos=0.5, above right] {1} (inbo1);
    \draw[-] (icebo1) -- node[pos=0.5, left] {1} (drebo1);
	\draw [->,>=stealth,orange] (drebo1) to[out=0,in=-90] node[pos=0.5, above left] {\tiny NextToken}(inbo1);
	\draw [->,>=stealth,blue] (icebo1) -- node[pos=0.5, above=0.1] {\tiny NextSibling}(inbo1);
	\draw [->,>=stealth,magenta] (drebo1) to[out=180,in=-115] node[pos=0.5, above right] {\tiny Ref}(varbo1);
	

	\node[base](csif1) at (4.5,8) {CompoundStmt};
	\node[base](if) at (4.5,6.5) {IfStmt};
	\node[base](bo) at (1.5,5) {BinaryOperator};
	\node[base](csif2) at (4.5,5) {CompoundStmt};
	\node[base](csif3) at (7.5,5) {CompoundStmt};
	
	\draw[-] (csif1) -- (if);
	\draw[-] (if) -- (bo);
	\draw[-] (if) -- (csif2);
	\draw[-] (if) -- (csif3);
	
	\draw[-implies,line width=1pt,double distance=5pt] (9,6.5) -- (11,6.5);
	
	\node[base](csif1) at (16.5,8) {CompoundStmt};
	\node[base](if) at (16.5,6.5) {IfStmt};
	\node[base](bo) at (13.5,5) {BinaryOperator};
	\node[base](csif2) at (16.5,5) {CompoundStmt};
	\node[base](csif3) at (19.5,5) {CompoundStmt};
	
	\draw[-] (csif1) -- node[pos=0.5, left] {50} (if);
	\draw[-] (if) -- node[pos=0.5, above left] {50} (bo);
	\draw[-] (if) -- node[pos=0.5, left] {25} (csif2);
	\draw[-] (if) -- node[pos=0.5, above right] {25} (csif3);
	\draw[->,>=stealth,thick,green] (bo) -- node[pos=0.5, above] {\tiny ConTrue} (csif2);
	\draw [->,>=stealth,red] (bo) to[out=-20,in=-160] node[pos=0.5, above] {\tiny ConFalse}(csif3);
	
	
	\node[base](csfor1) at (4.5,3) {CompoundStmt};
	\node[base](for) at (4.5,1.5) {ForStmt};
	\node[base](dsfor) at (0,0) {DeclStmt};
	\node[base](bofor) at (3,0) {BinaryOperator};
	\node[base](csfor2) at (6,0) {CompoundStmt};
	\node[base](usfor) at (9,0) {UnaryStmt};
	
	\draw[-] (csfor1) -- (for);
	\draw[-] (for) -- (dsfor);
	\draw[-] (for) -- (bofor);
	\draw[-] (for) -- (usfor);
	\draw[-] (for) -- (csfor2);
	
	\draw[-implies,line width=1pt,double distance=5pt] (9,1.5) -- (11,1.5);
	
	\node[base](csfor1) at (16.5,3) {CompoundStmt};
	\node[base](for) at (16.5,1.5) {ForStmt};
	\node[base](dsfor) at (12,0) {DeclStmt};
	\node[base](bofor) at (15,0) {BinaryOperator};
	\node[base](csfor2) at (18,0) {CompoundStmt};
	\node[base](usfor) at (21,0) {UnaryStmt};
	
	\draw[-] (csfor1) -- node[pos=0.5, left] {\small 1} (for);
	\draw[-] (for) -- node[pos=0.5, above left] {1} (dsfor);
	\draw[-] (for) -- node[pos=0.5, left] {50} (bofor);
	\draw[-] (for) -- node[pos=0.5, right] {50} (usfor);
	\draw[-] (for) -- node[pos=0.5, above right] {50} (csfor2);
	\draw [for] (dsfor) -- node[pos=0.5, above] {\tiny ForExec} (bofor);
	\draw [for] (bofor) -- node[pos=0.5, above] {\tiny ForExec} (csfor2);
	\draw [for] (csfor2) -- node[pos=0.5, above] {\tiny ForNext} (usfor);
	\draw [for] (usfor) to[out=-160,in=-20] node[pos=0.5, above] {\tiny ForNext}(bofor);
	
	\draw[draw=black,thick] (0,-1) rectangle (21,-3);
	\node[legend](ast) at (1.5,-1.5) {\small AST Edge};
	\node[legend](nxtTok) at (7,-1.5) {\small NextToken};
	\node[legend](ref) at (12.5,-1.5) {\small Reference};
	\node[legend](nxtSib) at (17.5,-1.5) {\small NextSibling};
	\node[legend](conF) at (1.5,-2.5) {\small ConFalse};
	\node[legend](conT) at (7,-2.5) {\small ConTrue};
	\node[legend](forEx) at (12.5,-2.5) {\small ForExec};
	\node[legend](forNxt) at (17.5,-2.5) {\small ForNext};
	
	\draw[-] (ast.west) -- ($(ast.west)-(.5,0)$);
	\draw[<-,>=stealth,thick, orange] (nxtTok.west) -- ($(nxtTok.west)-(.5,0)$);
	\draw[<-,>=stealth,thick,blue] (nxtSib.west) -- ($(nxtSib.west)-(.5,0)$);
	\draw[<-,>=stealth,thick,pink] (ref.west) -- ($(ref.west)-(.5,0)$);
	\draw[<-,>=stealth,thick,red] (conF.west) -- ($(conF.west)-(.5,0)$);
	\draw[<-,>=stealth,thick,green] (conT.west) -- ($(conT.west)-(.5,0)$);
	\draw[<-,>=stealth,thick,purple] (forEx.west) -- ($(forEx.west)-(.5,0)$);
	\draw[<-,>=stealth,thick,purple] (forNxt.west) -- ($(forNxt.west)-(.5,0)$);
\end{tikzpicture}
}
\caption{Modification to AST to create Augmented AST for ParaGraph}

\label{augmentedAST}
\end{figure*}


==> text/related_works.tex <==
\section{Related Works}

% PragML
% COMPOFF

A recent tool called BLISS~\cite{roy2021bliss} allows for auto-tuning parallel applications without the use of instrumentation or domain-specific knowledge.
This auto-tuner develops a variety of lightweight models with the aid of Bayesian optimization that can compete with the output quality of a complex, heavyweight Machine Learning (ML) model.
In the same context, Bayesian optimization is frequently used by other autotuners, including BOHB\cite{falkner2018bohb}, HiPerBOt~\cite{menon2020auto}, GPTune~\cite{liu2021gptune} and ytopt~\cite{wu2022autotuning}.
Unfortunately, due to their expensive evaluation functions, tuning large-scale HPC systems, which are becoming increasingly heterogeneous, complex, and expensive to evaluate, is still quite challenging.
These tools are unsuitable for our work due to their insufficient support for heterogeneous architectures, such as GPUs.

COMPOFF ~\cite{mishra2022compoff} provides a novel portable cost model that statically calculates the cost of OpenMP offloading on various architectures using a neural network model.
In this work we compare ParaGraph to COMPOFF since both predict the runtime of a kernel on a GPU.


